Active Linear Regression for $\ell_p$ Norms and Beyond

We study active sampling algorithms for linear regression, which aim to query only a few entries of a target vector $b\in\mathbb R^n$ and output a near minimizer to $\min_{x\in\mathbb R^d} \|Ax-b\|$, for a design matrix $A\in\mathbb R^{n \times d}$ and loss $\|\cdot\|$. For $p$ norm regression for any $0<p<\infty$, we give an algorithm based on Lewis weight sampling outputting a $(1+\epsilon)$-approximate solution using just $\tilde O(d/\epsilon^2)$ queries to $b$ for $p\in(0,1)$, $\tilde{O}(d/\epsilon)$ queries for $1<p<2$, and $\tilde{O}(d^{p/2}/\epsilon^p)$ queries for $2<p<\infty$. For $0<p<2$, our bounds are optimal up to log factors, settling the query complexity for this range. For $2<p<\infty$, our dependence on $d$ is optimal, while our dependence on $\epsilon$ is off by at most $\epsilon$, up to log factors. Our result resolves an open question of [CD21], who gave near optimal bounds for the $1$ norm, but required $d^2/\epsilon^2$ samples for $\ell_p$ regression with $1<p<2$, and gave no bounds for $2<p<\infty$ or $0<p<1$. We also give the first total sensitivity bound of $O(d^{\max\{1,p/2\}}\log^2n)$ for loss functions of degree $p$ polynomial growth, improving a result of [TMF20]. By combining this with our techniques for $\ell_p$ regression, we obtain an active regression algorithm making $\tilde O(d^{1+\max\{1,p/2\}}/\mathrm{poly}(\epsilon))$ queries for such loss functions, including the Tukey and Huber losses, answering another question of [CD21]. For the Huber loss, we further improve our bound to $\tilde O(d^{4-2\sqrt2}/\mathrm{poly}(\epsilon))$ samples. Our sensitivity bounds also have many applications, including Orlicz norm subspace embeddings, robust subspace approximation, and dimension reduction for smoothed $p$-norms. Finally, our active sampling results give the first sublinear time algorithms for Kronecker product regression under every $p$ norm.

==> active_regression/huber.tex <==
\section{Applications: Active Regression for the Huber Loss}\label{sec:huber}

Note that our sampling bound for general $M$-estimators from Section \ref{sec:active-m} is loose by a factor of $d$ compared to the corresponding bounds for $\ell_p$. This is due to the reliance on a na\"ive net argument rather than using the more efficient construction of \cite{BourgainLindenstraussMilman:1989,SchechtmanZvavitch:2001}. A natural question then is whether this can be improved or not, for loss functions other than the $\ell_p$ loss. We answer this in the affirmative for the important special case of the Huber loss.

More specificially, in this section, we obtain a sampling bound of
\[
    O(d^{4-2\sqrt 2}\poly(\eps^{-1},\log n))
\]
for subspace embeddings for the Huber loss, where $4 - 2\sqrt 2\approx 1.17157$, and 
\[
    O(d^{(1+\sqrt2)/2}\poly(\eps^{-1},\log n))
\]
for active regression for the Huber loss, where $(1+\sqrt2)/2\approx 1.20711$. These bounds are substantially better compared to the $O(d^{2}\poly(\eps^{-1},\log n))$ bound for other losses, which is obtained by a na\"ive Bernstein bound over a net. 

In what follows, we will first develop our recursive sampling algorithm for obtaining subspace embeddings for the Huber loss with the above sampling complexity, which can be used to obtain constant factor solutions in the active setting by Lemma \ref{lem:m-sensitivity-constant-factor-approx}. In Section \ref{sec:active-huber}, we then show how to modify our subspace embedding construction in order to get relative error bounds, again following Section \ref{sec:active-m}.

\subsection{Properties of the Huber Loss}

We first collect properties of the Huber loss needed to apply previous results for $M$-estimators. It is known that the Huber loss is polynomially bounded above with degree $2$ and constant $1$, and polynomially bounded below with degree $1$ and constant $1$. 

\begin{lemma}[Lemma 2.2 of \cite{ClarksonWoodruff:2015b}]
The Huber loss satisfies
\[
    \frac{y}{x} \leq \frac{H(y)}{H(x)} \leq \frac{y^2}{x^2}
\]
for all $y > x\geq 0$. 
\end{lemma}

This in turn implies that $H^{1/2}$ is subadditive, since it is known that polynomial growth with degree $1$ and constant $1$ implies subadditivity:

\begin{lemma}[Theorem 103 of \cite{HardyLittlewoodPolya:1973}]
Let $f:\mathbb R\to\mathbb R$. Suppose that $x\mapsto x^{-1}f(x)$ is decreasing, that is,
\[
    \frac{f(y)}{f(x)} \leq \frac{y}{x}
\]
for all $y > x$. Then, $f$ is subadditive. 
\end{lemma}

The following is a corollary that discretizes Lemma \ref{lem:generalized-huber-inequality}:

\begin{corollary}[Huber Inequality ver.\ 4]\label{cor:generalized-huber-inequality}
    Let $\bfy\in\mathbb R^n$ and let $\alpha \in [0,1/2]$ and $\gamma = n^{-\alpha}$ with $2/n \leq \gamma \leq 1$. Let
    \[
        T \supseteq \braces*{i\in[n] : H(\bfy_i) \leq \gamma \norm*{\bfy}_H^2},
    \]
    $\eps = c/\log n$ for some sufficiently small constant $c$, and let
    \[
        \mathcal I = \braces*{1, 1+\eps, 1+2\eps, \dots, 2 - \eps, 2} = \braces*{1 + \eps\cdot i : i\in \{0\}\cup[1/\eps]}. 
    \]
    Then, for some constant $c>0$, either
    \[
        \norm*{\bfy\mid_T}_H^2 \geq c\frac1{(\gamma n)^{3-2\sqrt 2}}\min_{p\in \mathcal I}\norm*{\bfy\mid_T}_p^p
    \]
    or
    \[
        \norm*{\bfy}_H^2 \geq c\gamma\min_{p\in\{1,2\}}\norm*{\bfy}_p^p
    \]
    where $3 - 2\sqrt 2 \approx 0.17157$.
\end{corollary}
\begin{proof}
    It was shown in the proof of Lemma \ref{lem:generalized-huber-inequality} that if $\norm*{\bfy}_1\geq 2n$, then $\norm*{\bfy}_H^2 = \Theta(\norm*{\bfy}_1)$, and if $\norm*{\bfy}_\infty \leq 1$, then $\norm*{\bfy}_H^2 = \norm*{\bfy}_2^2$. Thus, we may assume that all the entries of $\bfy$ are bounded by $O(n)$, and $\norm*{\bfy}_\infty \geq 1$. Note then that the entries that are at most $1/2n$ can make up at most an $\ell_p$ mass of $1/2$, and thus only affects the claimed inequality by a constant factor for any $p$. For all other entries, the magnitude is bounded below by $1/\poly(n)$ and above by $\poly(n)$, so an additive $O(1/\log n)$ difference in the exponent can only affect the bounds by a constant factor. We thus conclude the desired result. 
\end{proof}

\subsection{Net Arguments for the Huber Loss}\label{sec:huber-nets}

When constructing subspace embeddings for norms, it suffices to preserve the lengths of vectors on the unit normed sphere, by the scale invariance/homogeneity of norms. On the other hand, general $M$-estimators, including the Huber norm, do not necessarily satisfy scale invariance, which means that this strategy, as is, does not work. For the Huber norm, we show that for sufficiently small and sufficiently large scales, we have at least an $(1\pm\eps)$-approximate scale invariance, which allows us to obtain subspace embeddings by union bounding over finitely many scales. For all scales near $0$, this is because the Huber norm coincides with the $\ell_2$ norm. For larger scales, we show that the Huber norm is the $\ell_1$ norm up to $(1\pm\eps)$ factors. Then, the following result then shows that in order to prove subspace embeddings, it suffices to preserve the Huber norms of Huber balls at approximately $\log n$ radii.  

\begin{lemma}\label{lem:huber-multiple-nets}
Let $\bfA\in\mathbb R^{n\times d}$ and let $\mathcal V = \Span(\bfA)$. Let $\bfw\geq\mathbf{1}_n$ be a set of weights with 
\[
    W \coloneqq \norm*{\bfw}_\infty.
\]
Let $\eps>0$. Let 
\[
    \ell \coloneqq \log_2\sqrt{\frac{nW}{\eps}} = O\parens*{\log\frac{nW}{\eps}}.
\]
Suppose that
\[
    \norm*{\bfy}_{H,\bfw}^2 = (1\pm\eps)\norm*{\bfy}_H^2
\]
for every $\bfy\in \mathcal B_{\rho}^{H}$ for $\rho = 2^k$, for every $k\in[\ell]$. Then,
\[
    \norm*{\bfy}_{H,\bfw}^2 = (1\pm O(\eps))\norm*{\bfy}_H^2
\]
for all $\bfy\in\mathcal V$. 
\end{lemma}
\begin{proof}
    The intuition is as described above, and the details can be found in Appendix \ref{sec:huber-appendix}.
\end{proof}

\subsection{Compact Rounding for the Huber Loss}

In Section \ref{sec:huber-nets}, we have reduced our task to proving approximation guarantees for a small number of Huber spheres. We now focus on showing small sampling bounds for a single Huber sphere. 

Recall the net constructions of \cite{BourgainLindenstraussMilman:1989}, stated in Lemma \ref{lem:72}, as well as the compact rounding result of Lemma \ref{lem:round}. The following rounding lemma is implicit in the proof of Theorems 7.3 and 7.4 of \cite{BourgainLindenstraussMilman:1989}, which uses these net constructions. 

\begin{lemma}\label{lem:blm-compact-rounding}
Let $1\leq p < \infty$ and let
\[
    \mathcal B_p \coloneqq \braces*{\bfA\bfx : \norm*{\bfA\bfx}_p \leq 1}.
\]
Let $\eps \geq \gamma > 0$ and let $\mathcal N_\gamma$ be a standard $\gamma$-net on $\mathcal B_p$ with the $\ell_p$ norm, which has
\[
    \log \abs*{\mathcal N_\gamma} \leq O\parens*{d\log\frac{1}{\gamma}}
\]
by Lemma \ref{lem:standard-net}. Let $\bfy\in \mathcal N_\gamma$. Let $\ell = \ceil*{\log_{1+\eps}(2^{1/p}d^{1/p\lor 1/2})}$. Then, for $k\in[\ell]$, there exists a rounding
\[
    \tilde\bfy = \sum_{k=0}^\ell \tilde\bfy^{(k)}
\]
such that:
\begin{itemize}
    \item $\abs*{\tilde\bfy(i) - \bfy(i)} \leq 3\eps \abs*{\bfy(i)}$ for all $i\in[n]$
    \item $\abs*{\tilde\bfy^{(k)}(i)} \leq \bfW_{i,i}^{1/p}(1+\eps)^k$
    \item $\tilde\bfy^{(k)}$ for $0\leq k\leq \ell$ have disjoint supports
    \item each $\tilde\bfy^{(k)}$ is drawn from a set of vectors $\mathcal D_k$ with size at most
    \[
        \log\abs*{\mathcal D_k} \leq c(p)\frac{d}{\eps^{1+\beta}(1+\eps)^{\beta k}}\parens*{\log\frac{n}{\eps} + \log\frac1\gamma}
    \]
    where $\beta = (2\land p)$ and $c(p) = O\parens*{\max\braces*{p, \frac1{p-1}}}$. 
\end{itemize}
\end{lemma}

The lemma above is used to prove the following similar result for the Huber loss.

\begin{lemma}\label{lem:blm-net-for-huber}
    Let $\eps\in(0,1)$ and $\rho\geq 1$. Let $\bfA\in\mathbb R^{n\times d}$ and let $\bfy\in \mathcal S_\rho^H \subseteq \Span(\bfA)$. Let $\mathcal I\subset[1,2]$ be the set in the statement of Corollary \ref{cor:generalized-huber-inequality} and suppose that $\bfy$ satisfies
    \[
        \frac{\min_{p\in\mathcal I}\norm*{\bfy}_p^p}{\norm*{\bfy}_H^2} \leq \kappa_\bfy.
    \]
    Then, there exists a $p\in\mathcal I$, $\ell = O((\log d)/\eps^2)$, and a rounding
    \[
        \tilde\bfy = \sum_{k=0}^\ell \tilde\bfy^{(k)}
    \]
    such that:
    \begin{itemize}
        \item $\norm*{\tilde\bfy - \bfy}_H \leq O(\eps)\norm*{\bfy}_H$
        \item $H\parens*{\abs*{\tilde\bfy^{(k)}(i)}} \leq O(\kappa_\bfy)\parens*{\frac{\bfw_i^p(\bfA)}{d} + \frac1n} (1+\eps^2)^{pk}\norm*{\bfy}_H^2$
        \item $\tilde\bfy^{(k)}$ for $0\leq k\leq \ell$ have disjoint supports
        \item each $\tilde\bfy^{(k)}$ is drawn from a set of vectors $\mathcal D_k$ with size at most
        \[
            \log\abs*{\mathcal D_k} \leq O(1)\frac{d}{\eps^{2(1+p)}(1+\eps^2)^{pk}}\log\frac{n}{\eps}.
        \]
    \end{itemize}
\end{lemma}
\begin{proof}
    The proof is essentially by considering the $\ell_p$ \cite{BourgainLindenstraussMilman:1989} nets for $p\in\mathcal I$, and rounding $\bfy$ to the $\ell_p$ \cite{BourgainLindenstraussMilman:1989} net that minimizes $\norm*{\bfy}_p^p$. That is, for each vector $\bfy$, we choose that $p\in\mathcal I$ such that $\norm*{\bfy}_H^2$ is the closest to $\norm*{\bfy}_p^p$, and then round to this $\ell_p$ net. The details can be found in Appendix \ref{sec:huber-appendix}. 
\end{proof}

\subsection{Sampling Bounds}\label{subsec:huber-sampling-bounds}

With the above net results in hand, we can now complete the argument for one step of the sampling recursion. We start with a Bernstein bound using the net results. 

\begin{lemma}\label{lem:huber-bernstein}
    Let $\bfA\in\mathbb R^{n\times d}$ and let $\mathcal V = \Span(\bfA)$. Let $\eps\in(0,1)$ be an accuracy parameter, $\delta>0$ a failure rate parameter, $\rho \geq 1$ a Huber radius, and $\kappa\geq 1$ a distortion parameter. Let 
    \[
        m \coloneqq \frac{d}{\poly(\eps)}(\log^2 d)\parens*{\log\frac{n}{\eps}}\parens*{\log\frac{\log d}{\delta\eps}}.
    \]
    Let $\mathcal I$ be as in the statement of Corollary \ref{cor:generalized-huber-inequality}. Let $\bfw\geq \mathbf{1}_n$ be a set of weights chosen randomly so that
    \[
        \bfw_i \coloneqq \begin{cases}
            1/\bfp_i & \text{w.p. $\bfp_i$} \\
            0 & \text{otherwise}
        \end{cases}
    \]
    where
    \[
        \bfp_i \geq \min\braces*{1, m\cdot \kappa\bracks*{\frac1n + \sum_{p\in\mathcal I}\frac{\bfw_i^p(\bfA)}{d}}}
    \]
    Let
    \[
        S_\kappa \coloneqq \braces*{\bfy\in\mathcal V : \frac{\min_{p\in\mathcal I}\norm*{\bfy}_p^p}{\norm*{\bfy}_H^2}\leq \kappa}
    \]
    Then with probability at least $1 - \delta$, 
    \[
        \norm*{\bfy}_{H,\bfw} = (1\pm\eps)\norm*{\bfy}_H
    \]
    for all $\bfy\in \mathcal N\cap S_\kappa$, where $\mathcal N$ is an $\eps^2\rho$-net over $\mathcal S_\rho^H$ given by Lemma \ref{lem:blm-net-for-huber}, by setting $\eps$ in the lemma to $\eps^2$. 
\end{lemma}
\begin{proof}
    The proof is by applying Bernstein's inequality and union bounding over the net of Lemma \ref{lem:blm-net-for-huber}. The details can be found in Appendix \ref{sec:huber-appendix}. 
\end{proof}

We can now apply the result twice, once on all of the rows and once on only the set of rows with small Huber sensitivity, in order to obtain a sampling bound for preserving a Huber sphere at a single scale. 

\begin{lemma}\label{lem:huber-single-scale}
    Let $\bfA\in\mathbb R^{n\times d}$ and let $\mathcal V = \Span(\bfA)$. Let $\eps\in(0,1)$ be an accuracy parameter, $\delta>0$ a failure rate parameter, and $\rho \geq 1$ a Huber radius. Let $\beta = 3 - 2\sqrt 2$, $\gamma = n^{-\beta/(\beta+1)}$, and let
    \[
        T\coloneqq \braces*{i\in[n] : \bfs_i^H(\bfA) \leq \gamma}
    \]
    Let $\kappa \coloneqq O((\gamma n)^{\beta}) = O(\gamma^{-1})$ and let $\bfp$ be the sampling probabilities given by Lemma \ref{lem:huber-bernstein} for $\bfA$ and let $\bfq$ be the sampling probabilities given by Lemma \ref{lem:huber-bernstein} for $\bfA\mid_T$. Also let $\mathcal N$ and $\mathcal M$ be the corresponding nets. We then consider sampling probabilities $\bfr$ such that
    \[
        \bfr_i \coloneqq \begin{cases}
            1 & \text{if $i\in \overline T$} \\
            \min\braces*{\bfp_i + \bfq_i, 1} & \text{if $i\in T$}
        \end{cases}
    \]
    Let $\bfw\geq \mathbf{1}_n$ be a set of weights chosen randomly so that
    \[
        \bfw_i \coloneqq \begin{cases}
            1/\bfr_i & \text{w.p. $\bfr_i$} \\
            0 & \text{otherwise}
        \end{cases}
    \]
    Then,
    \[
        \norm*{\bfy}_{H,\bfw} = (1\pm O(\eps))\norm*{\bfy}_H
    \]
    for all $\bfy\in\mathcal S_\rho^H$ with probability at least $1 - \delta$. Furthermore,
    \[
        \E\nnz(\bfw) = O(\kappa m\log n) = O\parens*{\kappa d\poly\parens*{\frac{\log n}{\eps}}\log\frac1\delta}
    \]
    and
    \[
        \nnz(\bfw) = O\parens*{\E\nnz(\bfw) + \frac1\delta\log\frac1\delta}
    \]
    with probability at least $1 - \delta$. 
\end{lemma}
\begin{proof}
    By Corollary \ref{cor:generalized-huber-inequality}, we have that any vector $\bfy\in\mathcal S_\rho^H$ is either within an $\eps\norm*{\bfy}_H$ Huber distance away from some $\tilde\bfy\in\mathcal N$ or some $\tilde\bfy$ such that $\tilde\bfy\mid_T \in\mathcal M$. Then by Lemma \ref{lem:m-norm-net-to-sphere} we have that
    \[
        \norm*{\bfy}_{H,\bfw} = (1\pm O(\eps))\norm*{\bfy}_H
    \]
    for all $\bfy\in\mathcal S_\rho^H$, with probability at least $1 - 2\delta$.     
    
    Finally, letting $m$ be as in the statement of Lemma \ref{lem:huber-bernstein},
    \begin{align*}
        \E\nnz(\bfw) &= \sum_{i=1}^n \bfp_i + \bfq_i \\
        &\leq O(\kappa m)\parens*{\sum_{p\in\mathcal I}\bracks*{\frac1n + \sum_{i=1}^n \frac{\bfw_i^p(\bfA)}{d}}+\sum_{p\in\mathcal I}\bracks*{\frac1n + \sum_{i\in T} \frac{\bfw_i^p(\bfA\mid_T)}{d}}} \\
        &= O(\kappa m\abs*{\mathcal I}) = O(\kappa m\log n)
    \end{align*}
    since Lewis weights sum to $d$. If $\E\nnz(\bfw) \leq O(\log\frac1\delta)$, then by Markov's inequality,
    \[
        \nnz(\bfw) \leq O\parens*{\frac1\delta \log\frac1\delta}
    \]
    with probability at least $1 - \delta$. Otherwise, by Bernstein's inequality,
    \[
        \nnz(\bfw) = \Theta(\E\nnz(\bfw))
    \]
    with probability at least $1 - \delta$. 
\end{proof}

Finally, we assemble the previous lemmas into Algorithm \ref{alg:unweighted-huber-subspace-embedding}, whose guarantee is proven in Theorem \ref{thm:n13d-huber-sampling}. 

\begin{algorithm}
	\caption{Unweighted Huber subspace embedding}
	\textbf{input:} Matrix $\bfA \in \R^{n \times d}$. \\
	\textbf{output:} Weights $\bfw$.
	\begin{algorithmic}[1] % The number tells where the line numbering should start
        \State $\beta\gets 3 - 2\sqrt 2$, $\gamma\gets n^{-\beta/(1+\beta)}$, $m\gets d\poly((\log n)/\eps)$
		\State Compute approximate Huber sensitivities $\tilde\bfs_i^H(\bfA)$ with Algorithm \ref{alg:m-estimator-alg-sensitivity} with $\tau = \gamma n$
        \State $T\gets \{i\in[n] : \tilde\bfs_i^H(\bfA)\geq \gamma\}$
        \State Set $\bfw_i = 1$ for every $i\in T$
        \State $\mathcal I\gets\{1+(c/\log n)\cdot j : j\in[(\log n)/c]\cup\{0\}\}$
        \State Compute approximate Lewis weights $\tilde\bfw_i^p(\bfA)$ with Theorem \ref{thm:cohen-peng-fast-lewis-weights} for every $p\in\mathcal I$
        \State Compute approximate Lewis weights $\tilde\bfw_i^p(\bfA\mid_T)$ with Theorem \ref{thm:cohen-peng-fast-lewis-weights} for every $p\in\mathcal I$
        \For{$i\in T$}
        \State Let $\bfp_i = \min\{1,\gamma^{-1}m(1/n + \sum_{p\in\mathcal I}\tilde\bfw_i^p(\bfA)/d) + \sum_{p\in\mathcal I}\tilde\bfw_i^p(\bfA\mid_T)/d)\}$
        \State Set $\bfw_i = 1/\bfp_i$ with probability $\bfp_i$ and $0$ otherwise.
        \EndFor
        \State \Return $\bfw$
	\end{algorithmic}\label{alg:unweighted-huber-subspace-embedding}
\end{algorithm}

\begin{theorem}\label{thm:n13d-huber-sampling}
    Let $\bfA\in\mathbb R^{n\times d}$ and let $\mathcal V = \Span(\bfA)$. Let $\eps>0$ and $\delta > 0$. Let $\bfw\geq\mathbf{1}_n$ be a set of weights chosen at random according to Lemma \ref{lem:huber-single-scale}, where we set $\delta$ in the lemma statement to $\delta/100\ell$, where
    \[
        \ell \coloneqq \log_2\sqrt{\frac{2n^2}{\eps}} = \Theta\parens*{\log\frac{n}{\eps}}
    \]
    as in the statment of Lemma \ref{lem:huber-multiple-nets} with $W = 2n$. Let $\beta = 3 - 2\sqrt 2$ and $\gamma = n^{-\beta/(\beta+1)}$. Then,
    \[
        \norm*{\bfy}_{H,\bfw}^2 = (1\pm O(\eps))\norm*{\bfy}_H^2
    \]
    for all $\bfy\in\mathcal V$ and
    \[
        \E\nnz(\bfw) = O\parens*{\gamma^{-1}d\poly\parens*{\frac{\log n}{\delta\eps}}}.
    \]
    Furthermore,
    \[
        \nnz(\bfw) = O\parens*{\E\nnz(\bfw) + \frac1\delta\log\frac1\delta}
    \]
    with probability at least $1 - \delta$. Furthermore, Algorithm \ref{alg:unweighted-huber-subspace-embedding} runs in time
    \[
        O\parens*{(\nnz(\bfA) + d^{(1+\beta)\omega})(\log^2 n)\log\frac1\delta}.
    \]
\end{theorem}
\begin{proof}
    We first identify the rows with Huber sensitivity at least $\gamma$. By running Theorem \ref{thm:m-estimator-alg} $\log(1/\delta)$ times with $\tau = \gamma n = n^{1/(\beta+1)}$, we can boost the success probability to $1-\delta$ to find sensitivity upper bounds that sum to
    \[
        O\parens*{d(\log^2 n)\log\frac1\delta}
    \]
    in time
    \[
        O\parens*{\bracks*{\nnz(\bfA)\log^2 n + n^{1/(\beta+1)}T\log n}\log\frac1\delta}.
    \]
    for $T = O(d^{\omega}\log^2 d)$ by Theorem \ref{thm:cohen-peng-fast-lewis-weights}. This is $O(\nnz(\bfA)\log^2 n)$ time for $T \leq n^{1/(\beta+1)}$ and $O(T^{1+\beta}\log^2 n)$ time for $T \geq n^{1/(\beta+1)}$. Then, we may find a superset of rows with Huber sensitivity at least $\gamma$ of size at most $O\parens*{\gamma^{-1}d(\log^2 n)\log\frac1\delta}$. We may also approximate the $\ell_1$ and $\ell_2$ Lewis weights in time $O([\nnz(A) + T]\log\frac1\delta)$ by Theorem \ref{thm:cohen-peng-fast-lewis-weights}. 

    By applying Lemma \ref{lem:huber-single-scale} with the $\delta$ in the lemma set to $\delta/100\ell$, we can union bound over the $\ell$ spheres $\mathcal S_\rho^H$ as given in Lemma \ref{lem:huber-multiple-nets} with probability at least $1 - \delta$. Then, with probability at least $1 - \delta$,
    \[
        \norm*{\bfy}_{H,\bfw}^2 = (1\pm O(\eps))\norm*{\bfy}_H^2
    \]
    for all $\bfy\in\mathcal V$ by Lemma \ref{lem:huber-multiple-nets} and the guarantees on $\nnz(\bfw)$ follow from Lemma \ref{lem:huber-single-scale}.
\end{proof}

\subsection{Subspace Embeddings via Recursive Sampling}

For large $n$, a bound of $\tilde O(n^{\beta/(\beta+1)}d)$ with $\beta = 3-2\sqrt 2$ of Theorem \ref{thm:n13d-huber-sampling} is much worse than the previous $O(d^2\poly\log(n))$ bound. However, by applying Theorem \ref{thm:n13d-huber-sampling} \emph{after} reducing the number of rows to $O(d^2\poly\log(n))$, we can obtain a sampling bound of roughly $O(d^{2\beta/(\beta+1)}\poly\log(n))$, where $1 + 2\beta/(\beta+1)\approx 1.29289$. Furthermore, by recursively applying this procedure, we can improve the dependence on $d$ to $d^{1+\beta} = d^{4-2\sqrt 2}$ after only $O(\log\log(d\log n))$ many iterations, where $4-2\sqrt 2\approx 1.17157$.

We first describe how to perform one step of the recursive sampling procedure. 

\begin{algorithm}
	\caption{Weighted Huber subspace embedding}
	\textbf{input:} Matrix $\bfA \in \R^{n \times d}$ and weights $\bfw$. \\
	\textbf{output:} Weights $\bfw'$.
	\begin{algorithmic}[1] % The number tells where the line numbering should start
        \For{$j\in[O(\log(1+\norm*{\bfw}_\infty)/\eps)]$}
        \State $T_j\gets\{i\in[n] : (1+\eps)^{j-1} \leq \bfw_i < (1+\eps)^j\}$
        \State Run Algorithm \ref{alg:unweighted-huber-subspace-embedding} on $\bfA\mid_{T_j}$ to obtain weights $\bfw^{(j)}$
        \State Set $\bfw'_i = (1+\eps)^j\bfw^{(j)}_i$ for $i\in T_j$
        \EndFor
        \State \Return $\bfw'$
	\end{algorithmic}\label{alg:weighted-huber-subspace-embedding}
\end{algorithm}

\begin{lemma}\label{lem:huber-one-recursive-step}
    Let $\bfw\geq\mathbf{1}_n$ be a set of weights. Let $\eps > 0$ and $\delta > 0$. Let $\beta=3-2\sqrt 2$. Then, using Algorithm \ref{alg:weighted-huber-subspace-embedding}, we may construct $\bfw'\geq\mathbf{1}_n$ such that with probability at least $1 - \delta$:
    \begin{itemize}
        \item $\norm*{\bfw'}_\infty \leq n\norm*{\bfw}_\infty$
        \item \[
            \nnz(\bfw') \leq O\parens*{(\log\norm*{\bfw}_\infty) n^{\beta/(\beta+1)}d\poly\parens*{\frac{\log n}{\eps}} + \frac{\log^2\norm*{\bfw}_\infty}{\eps^2\delta}\log\frac{\log\norm*{\bfw}_\infty}{\eps\delta}}
        \]
        \item $\norm*{\bfA\bfx}_{H,\bfw'}^2 = (1\pm 3\eps) \norm*{\bfA\bfx}_{H,\bfw}^2$ for all $\bfx\in\mathbb R^d$
        \item The algorithm runs in time at most
        \[
            O\parens*{\nnz(\bfA)(\log^3 n)\log\frac1\delta + d^{(1+\beta)\omega}\poly\parens*{\frac{\log(n/\delta)}{\eps}}}
        \]
    \end{itemize}
\end{lemma}
\begin{proof}
    The proof breaks up the weights into $O(\log n/\eps)$ levels and applies Theorem \ref{thm:n13d-huber-sampling} on each level set. The details can be found in Appendix \ref{sec:huber-appendix}. 
\end{proof}


Now note that as long as we apply this recursion at most $\log n$ times, the number of rows decreases as $m \to O(m^{\beta/(\beta+1)}d\poly((\log n) / \eps))$ at each iteration. The closed form solution to this can be found via the following recurrence:

\begin{lemma}\label{lem:affine-recurrence}
    Suppose that $(a_i)_{i=0}^\infty$ satisfies the recurrence
    \[
        a_{i+1} = \lambda a_i + b
    \]
    for some $b > 0$ and $\lambda\in(0,1)$. Then,
    \[
        a_i = \frac{1}{1-\lambda} \parens*{b - \lambda^{i}\parens*{b - (1-\lambda) a_0}}
    \]
\end{lemma}
\begin{proof}
    The proof can be found in Appendix \ref{sec:huber-appendix}. 
\end{proof}


By applying the above lemma on the logarithm of the number of rows after the $i$th recursive application of row sampling, where $b$ corresponds to $\log(d\poly((\log n) / \eps)))$, we obtain the following algorithm and theorem:

\begin{algorithm}
	\caption{Recursive Huber subspace embedding}
	\textbf{input:} Matrix $\bfA \in \R^{n \times d}$, weights $\bfw$ (defaulted to $\mathbf{1}_n$). \\
	\textbf{output:} Weights $\bfw''$.
	\begin{algorithmic}[1] % The number tells where the line numbering should start
        \State $\beta\gets3-2\sqrt 2$
        \If{$\nnz(\bfw) \leq O(d^{1+\beta}\poly((\log n)/\eps))$}
            \State \Return $\bfw$
        \EndIf
        \State Obtain weights $\bfw'$ by running Algorithm \ref{alg:weighted-huber-subspace-embedding} on $\bfA$ with weights $\bfw$
        \State Obtain weights $\bfw''$ by recursively running Algorithm \ref{alg:huber-subspace-embedding} on $\bfA$ with weights $\bfw'$
        \State \Return $\bfw''$
	\end{algorithmic}\label{alg:huber-subspace-embedding}
\end{algorithm}

\begin{theorem}[Huber Subspace Embedding]\label{thm:huber-subspace-embedding}
    There is an algorithm (Algorithm \ref{alg:huber-subspace-embedding}) which, with probability $99/100$, computes a set of weights $\bfw\geq\mathbf{1}_n$ with
    \[
        \nnz(\bfw) \leq O(d^{4-2\sqrt 2}\poly((\log n)/\eps))
    \]
    such that $\norm*{\bfA\bfx}_{H,\bfw'}^2 = (1\pm 3\eps) \norm*{\bfA\bfx}_{H,\bfw}^2$ for all $\bfx\in\mathbb R^d$, and runs in time
    \[
            O\parens*{\nnz(\bfA)(\log^3 n)(\log^2\log n) + d^{\omega(4-2\sqrt 2)}\poly\parens*{\frac{\log(n)}{\eps}}}.
    \]
\end{theorem}
\begin{proof}
We apply Lemma \ref{lem:huber-one-recursive-step} for $O(\log\log n)$ recursive steps with $\delta = O(1/\log\log n)$ so that we have a sequence of upper bounds $m_i$ on the number of rows such that, for $\beta = 3-2\sqrt 2$,
\[
    m_i = O\parens*{m_{i-1}^{\beta/(\beta+1)}d \poly\parens*{\frac{\log n}{\eps}}}.
\]
Note then that $a_i\coloneqq \log m_i$ satisfies
\[
    a_i = \frac{\beta}{\beta+1} a_{i-1} + b
\]
for
\[
    b = \log\bracks*{O\parens*{d\poly\parens*{\frac{\log n}{\eps}}}}.
\]
The closed form solution for this is given in Lemma \ref{lem:affine-recurrence}. Note that if $i$ satisfies
\[
    \parens*{\frac{\beta}{\beta+1}}^{i}\parens*{b + \frac{1}{\beta+1} a_0} \leq \frac1{\log b}
\]
then
\[
    a_i = (1+\beta) b \pm \frac1{\log b}
\]
and thus the number of rows is at most 
\[
    m_i = \exp(a_i) = O(\exp(b)^{1+\beta}) = O(d^{1+\beta}\poly((\log n)/\eps)) =  O(d^{4-2\sqrt2}\poly((\log n)/\eps)).
\]
This only requires $i$ at most $O(\log(b + a_0)) = O(\log\log n)$ iterations. 
\end{proof}


\subsection{Active Regression Algorithms}\label{sec:active-huber}

As noted before, Theorem \ref{thm:huber-subspace-embedding} gives constant factor solutions in the active regression setting, by Lemma \ref{lem:m-sensitivity-constant-factor-approx}. We now discuss how to build on this result to obtain a relative error solution, using the more refined techniques of Section \ref{subsec:relative-error-lp}. Our dependence on $d$ will be slightly worse than the that obtained in the non-active setting in Theorem \ref{thm:huber-subspace-embedding}. This is due to a difficulty in adapting the technique of storing large Huber sensitivities to the active setting.

Our main result of this section is the following:

\begin{theorem}[Main Result for Huber Active Regression]\label{thm:active-huber}
    Let $\bfA \in \R^{n \times d}$, $\bfb \in \R^n$. Then, with probability at least $99/100$, Algorithm \ref{alg:huber-active} returns a $\tilde\bfx$ satisfying 
    \[
        \norm{\bfA\tilde \bfx - \bfb}_H \le (1+\epsilon) \cdot \min_\bfx\norm*{\bfA\bfx - \bfb}_H
    \]
    Furthermore, the algorithm reads at most $d^{(1+\sqrt 2)/2}\poly(\log n,\eps^{-1})$ entries of $\bfb$. 
\end{theorem}

\begin{algorithm}
	\caption{Active regression with the Huber loss}
	\textbf{input:} Matrix $\bfA \in \R^{n \times d}$, $\bfb\in\mathbb R^n$. \\
	\textbf{output:} Approximate solution $\tilde\bfx\in\R$ to $\min_\bfx\norm*{\bfA\bfx-\bfb}_H$.
	\begin{algorithmic}[1] % The number tells where the line numbering should start
        \State Let $\bfw$ be generated by Algorithm \ref{alg:huber-subspace-embedding}
        \State Let $\bfx_c$ be an approximate minimizer $\norm*{\bfA\bfx_c-\bfb}_{H,\bfw} \leq (1+\gamma)\min_\bfx\norm*{\bfA\bfx-\bfb}_{H,\bfw}$ for $\gamma = O(1)$
        \State Set $\bfz\gets\bfb - \bfA\bfx_c$ 
        \State Let $\bfw'$ be generated by Algorithm \ref{alg:huber-recursive-active} \label{line:eps-huber-subspace-embedding}
        \State Let $\bar\bfx$ be an approximate minimizer $\norm*{\bfA\bar\bfx-\bfz}_{H,\bfw'} \leq (1+\eps)\min_\bfx\norm*{\bfA\bfx-\bfz}_{H,\bfw'}$
        \State \Return $\tilde\bfx = \bar\bfx + \bfx_c$
	\end{algorithmic}\label{alg:huber-active}
\end{algorithm}

We first obtain an analog of Lemmas \ref{lem:clip} and \ref{lem:clip2}, mirroring some of the logic from Lemma \ref{lem:m-active-regression-relative-error-approximation}.

\begin{lemma}\label{lem:huber-clip}
Let $\bfA\in\R^{n\times d}$ and let $\bfz\in\mathbb R^n$. Let $\bfw\geq\mathbf{1}_n$ be a set of weights. Suppose that $\overline{\bfs_i}^{H,\bfw}(\bfA)\geq\bfs_i^{H,\bfw}(\bfA)$ is any upper bound on the Huber sensitivities\footnote{We will set $\overline{\bfs_i}^{H,\bfw}(\bfA)$ to be a function of $\tilde\bfs_i^{H,\bfw}(\bfA)$ (constant factor approximations to the Huber sensitivities), hence the different notation.}. Let $\OPT \coloneqq \min_\bfx\norm*{\bfA\bfx - \bfz}_{H,\bfw}$. Suppose that $\bfz$ satisfies $\norm*{\bfz}_{H,\bfw} = O(\OPT)$. Let
\[
    \mathcal B\coloneqq\braces*{i\in[n] : \bfw_i H(\bfz_i) \geq \frac{\overline{\bfs_i}^{H,\bfw}(\bfA)}{\eps^2}\OPT^2}
\]
Let $\bar\bfz\in\mathbb R^n$ be equal to $\bfz$, but with all entries in $\mathcal B$ set to $0$. Then, for all $\bfx\in\mathbb R^d$ with $\norm*{\bfA\bfx}_{H,\bfw} = O(\OPT)$,
\[
    \abs*{\norm*{\bfA\bfx-\bfz}_{H,\bfw}^2-\norm*{\bfA\bfx-\bfz}_{H,\bfw}^2 - \norm*{\bfz-\bar\bfz}_{H,\bfw}^2} = O(\eps)\OPT^2.
\]
\end{lemma}
\begin{proof}
    For any $\bfx\in\R^d$ such that $\norm*{\bfA\bfx}_{H,\bfw} = O(\OPT)$ and any $i\in\mathcal B$,
    \[
        \bfw_i H([\bfA\bfx](i)) \leq \overline{\bfs_i}^{H,\bfw}(\bfA)\norm*{\bfA\bfx}_{H,\bfw}^2 \leq \overline{\bfs_i}^{H,\bfw}(\bfA)O(\OPT^2) \leq O(\eps^2)\bfw_i H(\bfz_i).
    \]
    Then, for $i\in\mathcal B$, we have by the Huber triangle inequality (see Lemma \ref{lem:triangle-inequality-m}) that
    \begin{align*}
        \bfw_i H([\bfA\bfx](i)-\bfz(i)) - \bfw_i H([\bfA\bfx](i)-\bar\bfz(i)) &= \bfw_i H([\bfA\bfx](i)-\bfz(i)) - \bfw_i H([\bfA\bfx](i)) \\
        &= \bfw_i\parens*{H^{1/2}(\bfz(i))\pm H^{1/2}([\bfA\bfx](i))}^2 - \bfw_i H([\bfA\bfx](i)) \\
        &= (1\pm O(\eps))\bfw_i H(\bfz_i)
    \end{align*}
    Thus, letting $C = \sum_{i\in\mathcal B}\bfw_i H\parens*{\bfz(i)} = \norm*{\bfz - \bar\bfz}_{H,\bfw}^2$ and using that $\norm*{\bfz - \bar\bfz}_{H,\bfw}^2 \leq \norm*{\bfz}_{H,\bfw}^2 = O(\OPT^2)$,
    \[
        \abs*{\norm*{\bfA\bfx-\bfz}_{H,\bfw}^2 - \norm*{\bfA\bfx-\bar\bfz}_{H,\bfw}^2 - C} \leq O(\eps)\norm*{\bfz-\bar\bfz}_{H,\bfw}^2 = O(\eps)\OPT^2.
    \]
\end{proof}

Next, we show that our Huber subspace embedding algorithm approximately preserves Huber norms $\norm*{\bfA\bfx-\bar\bfz}_{H,\bfw}^2$ for all $\bfx\in\mathbb R^d$ such that $\norm*{\bfA\bfx}_{H,\bfw} = O(\OPT)$. We start by showing the result for one step of the unweighted algorithm of Algorithm \ref{alg:unweighted-huber-active}, which is the bulk of the work for this section.

\begin{algorithm}
	\caption{Unweighted Huber sampling}
	\textbf{input:} Matrix $\bfA \in \R^{n \times d}$. \\
	\textbf{output:} Weights $\bfw$.
	\begin{algorithmic}[1] % The number tells where the line numbering should start
        \State $\kappa\gets n^{3-2\sqrt 2}$, $m\gets d\poly((\log n)/\eps)$
		\State Compute approximate Huber sensitivities $\tilde\bfs_i^H(\bfA)$ with Algorithm \ref{alg:m-estimator-alg-sensitivity} with $\tau = \gamma n$
        \State $\mathcal I\gets\{1+(c/\log n)\cdot j : j\in[(\log n)/c]\cup\{0\}\}$
        \State Compute approximate Lewis weights $\tilde\bfw_i^p(\bfA)$ with Theorem \ref{thm:cohen-peng-fast-lewis-weights} for every $p\in\mathcal I$
        \For{$i\in [n]$}
        \State Let $\bfp_i = \min\{1,\kappa\cdot m(1/n + \tilde\bfs_i^H(\bfA)/d + \sum_{p\in\mathcal I}\tilde\bfw_i^p(\bfA)/d)\}$
        \State Set $\bfw_i = 1/\bfp_i$ with probability $\bfp_i$ and $0$ otherwise.
        \EndFor
        \State \Return $\bfw$
	\end{algorithmic}\label{alg:unweighted-huber-active}
\end{algorithm}

\begin{lemma}\label{lem:huber-additive2}
    Consider the setting of Lemma \ref{lem:huber-clip}. Suppose that $\bfw$ is obtained by performing one step of Algorithm \ref{alg:unweighted-huber-active}. Then with probability at least $1-\delta$, for all $\bfx\in\mathbb R^{d}$ with $\norm*{\bfA\bfx}_{H} = O(\OPT)$,
    \begin{equation}\label{eq:huber-additive2-guarantee}
        \abs*{\norm*{\bfA\bfx-\bar\bfz}_{H}^2 - \norm*{\bfA\bfx-\bar\bfz}_{H,\bfw}^2} = O(\eps)\cdot\OPT^2.
    \end{equation}
\end{lemma}
\begin{proof}
    We combine the $\ell_p$ compact rounding technique for the active setting in Lemma \ref{lem:round} with our Huber subspace embedding techniques from Section \ref{subsec:huber-sampling-bounds}. 

    Note that we only need to provide Huber norm preservation guarantees for a single scale of Huber radius $\rho = O(\OPT)$ for this lemma, as opposed to $O(\log n)$ scales for the Huber subspace embedding result. Furthermore, by Lemma \ref{lem:m-norm-net-to-sphere}, it suffices to show the approximation guarantee for every $\bfy\in\mathcal N\cup(\mathcal N-\bar\bfz)$, where $\mathcal N$ is an $O(\eps^2\rho)$-cover of $\mathcal B_\rho^{H,\bfw}$. We have already shown in Theorem \ref{thm:huber-subspace-embedding} the preservation of $\norm*{\bfy}_{H,\bfw}^2$ for every $\bfy$ in $\mathcal N$, so we focus on showing the preservation of $\norm*{\bfy}_{H,\bfw}^2$ for every $\bfy\in\mathcal N-\bar\bfz$, which is similar but requires a slightly more involved argument to handle the $\bar\bfz$ translation.

    We start off with the following claim, which is the active version of Lemma \ref{lem:blm-net-for-huber} and the Huber version of Lemma \ref{lem:round}.

    \begin{claim}\label{clm:huber-compact-rounding}
        Let $\mathcal I\subset[1,2]$ be the set in the statement of Corollary \ref{cor:generalized-huber-inequality}. Suppose that $\overline{\bfs_i}^{H,\bfw}(\bfA)\geq\bfs_i^{H,\bfw}(\bfA)$ is an upper bound on the Huber sensitivities such that
        \begin{equation}\label{eq:huber-lp-sensitivity-bound}
            \bfw_i^p(\bfA) \leq \overline{\bfs_i}^{H,\bfw}(\bfA)
        \end{equation}
        for every $p\in\mathcal I$. Let $\bfv\in\mathbb R^n$ be a target vector satisfying
        \[
            H(\bfv(i)) \leq \frac{\overline{\bfs_i}^H(\bfA)}{\eps^4}\OPT^2
        \]
        for each $i\in[n]$.
        Let $\bfr = \bfy - \bfv\in (\mathcal B_\rho^H - \bfv)$ for $\rho = O(\OPT)$. Suppose that $\bfy$ satisfies
        \[
            \frac{\min_{p\in\mathcal I}\norm*{\bfy}_p^p}{\norm*{\bfy}_H^2} \leq \kappa.
        \]
        Then, there exists a $p\in\mathcal I$, $\ell = O((\log d)/\eps^2)$, and a rounding $\bfr' = \bfe + \sum_{k=0}^\ell \bfd_k$ such that:
        \begin{itemize}
            \item $\norm*{\bfr' - \bfr}_H \leq O(\eps)\OPT$
            \item $H\parens*{\abs*{\bfd_k(i)}} \leq O(\kappa)\frac{\overline{\bfs_i}^H(\bfA)\cdot(1+\eps^2)^{pk}}{\eps^4\cdot d}\OPT^2$
            \item $\bfe, \bfd_0, \bfd_1, \dots, \bfd_\ell$ have disjoint supports
            \item $\bfe$ is a single fixed vector with $H(\abs{\bfe(i)}) \leq O(\kappa)\frac{\overline{\bfs_i}^H(\bfA)}{\eps^4\cdot d}\OPT^2$
            \item each $\bfd_k$ is drawn from a set of vectors $\mathcal D_k$ with size at most
            \[
                \log\abs*{\mathcal D_k} \leq O(1)\frac{d}{\eps^{2(1+p)}(1+\eps^2)^{pk}}\log\frac{n}{\eps}.
            \]
        \end{itemize}
    \end{claim}
    \begin{proof}
        Let $p\in\mathcal I$ be the $p$ achieving the minimum in Corollary \ref{cor:generalized-huber-inequality} for $\bfy$. We then define the $\ell$ nets $\mathcal N_k$ for $k\in[\ell]$ and the index sets $C_{k,\bfy}$ and $D_{k,\bfy}$ exactly as in Claim \ref{clm:blm-index-sets}, with $\eps$ set to $\eps^2$. We also explicitly keep track of the scaling without assuming that $\OPT = \Theta(1)$, as the Huber loss is not scale invariant. We then define a slightly different version of the index sets for the target vector $\bfv$ by modifying Claim \ref{clm:partition} as follows:

        \begin{claim}[Huber index sets for $\bfv$]\label{clm:huber-partition}
            Define the following sets (Note that the $\eps$ are set to $\eps^2$ compared to Claim \ref{clm:partition}):
        \begin{align*}
            B_{k,\bfy} &\coloneqq \braces*{i \in D_{k,\bfy}: H(\bfv(i)) \le \kappa\frac{\overline{\bfs_i}^H(\bfA) \cdot (1+\epsilon^2)^{p(k+2)}}{\epsilon^4 \cdot d}\OPT^2} \tag{$k\in[\ell]\cup\{0\}$} \\
            H_k &\coloneqq \braces*{i\in[n]: \kappa\frac{\overline{\bfs_i}^H(\bfA)\cdot (1+\epsilon^2)^{p(k+1)}}{\epsilon^4 \cdot d}\OPT^2 < H(\bfv(i))\le \kappa\frac{\overline{\bfs_i}^H(\bfA) \cdot (1+\epsilon^2)^{p(k+2)}}{\epsilon^4 \cdot d}\OPT^2 } \tag{$k\in[\ell]$} \\
            H_B &\coloneqq \braces*{ i\in[n]: H(\bfv(i)) > \kappa\frac{\overline{\bfs_i}^H(\bfA) \cdot (1+\epsilon^2)^{p(\ell+2)}}{\epsilon^4 \cdot d}\OPT^2 } \\
            G_{k,\bfy} &\coloneqq H_{k} \setminus \bigcup_{k' \ge k} C_{k',\bfy}
        \end{align*}
        Then, $B_{0,\bfy},\ldots,B_{\ell,\bfy},G_{1,\bfy},\ldots,G_{\ell,\bfy}, H_B$ form a partition of $[n]$.
        \end{claim}
        \begin{proof}
        The proof is nearly identical to that of Claim \ref{clm:partition}, so we give a brief summary. Define $H_{0} = \{i: H(\bfv(i)) \le \kappa\frac{\overline{\bfs_i}^H(\bfA) \cdot (1+\epsilon^2)^{2p}}{\epsilon^4 \cdot d}\OPT^2 \}$, so that $H_B \cup \bigcup_{k=0}^\ell H_{k} = [n]$ is a partition the range of all possible $H(\bfv(i))$ values. Then, $H_k$ can be furthered partitioned into the indices that lie in some $\bigcup_{k'\geq k}C_{k,\bfy}$, or those that are not in any $\bigcup_{k'\geq k} C_{k',\bfy}$. Those that lie in some $\bigcup_{k'\geq k}C_{k,\bfy}$ are then regrouped into the $B_{k,\bfy}$, which is also a valid partition by definition of the $D_{k,\bfy}$.
        \end{proof}

        Finally, as in Claim \ref{clm:infty}, we obtain a rounding $\bfr'$ for $\bfr = \bfy - \bfv$ via
        \[
            \bfr' = \bfe + \sum_{k=0}^\ell \bfd_k
        \]
        where $\bfe$ and $\bfd_k$ are defined exactly as in Equation \eqref{eq:active-rounding-definition}, but with definitions of $B_{k,\bfy}$, $H_B$, and $G_{k,\bfy}$ as in Claim \ref{clm:huber-partition}. As in Claim \ref{clm:infty}, we have that
        \[
            \abs*{\bfr(i) - \bfr'(i)} \leq O(\eps^2)(\abs*{\bfy(i)}+\abs*{\bfv(i)}).
        \]
        Indeed, $\bfr(i) = \bfr'(i)$ for $i\in B_{0,\bfy}$, $\abs*{\bfr(i) - \bfr'(i)} \leq O(\eps^2)\abs*{\bfy(i)}$ for $i\in B_{k,\bfy}$ by Equation \eqref{yi_bound}, and for $i\in G_{k,\bfy}$ we have
        \begin{align*}
            H(\abs*{\bfy(i)}) &\leq \abs*{\bfy(i)}^p \tag{$p\in[1,2]$} \\
            &\leq \frac{\bfw_i^p(\bfA)\cdot (1+\eps^2)^{p(k+2)}}{d}\norm*{\bfy}_p^p \tag{$i\notin \bigcup_{k'\geq k}C_{k',\bfy}$} \\
            &\leq \kappa\frac{\bfw_i^p(\bfA)\cdot (1+\eps^2)^{p(k+2)}}{d}\norm*{\bfy}_H^2\\
            &\leq \kappa\frac{\overline{\bfs_i}^H(\bfA)\cdot (1+\eps^2)^{p(k+2)}}{d}\cdot O(\OPT^2) \tag{Equation \eqref{eq:huber-lp-sensitivity-bound}} \\
            &\leq O(\eps^4)H(\bfv(i)) \tag{$i\in H_k$}
        \end{align*}
        and similarly for $i\in H_B$.
        
        We then have that
        \begin{align*}
            \sum_{i=1}^n H(\abs*{\bfr'(i)-\bfr(i)}) &\leq \sum_{i=1}^n H(\eps^2(\abs{\bfy(i)} + \abs*{\bfv(i)})) \tag{monotonicity} \\
            &\leq O(\eps^2)\sum_{i=1}^n H(\abs{\bfy(i)} + \abs*{\bar\bfz(i)}) \tag{at least linear growth} \\
            &= O(\eps^2)(\norm*{\bfy}_{H,\bfw} + \norm*{\bar\bfz}_{H,\bfw})^2 = O(\eps^2)\OPT^2 \tag{triangle inequality}
        \end{align*}
        so $\norm*{\bfr'-\bfr}_H \leq O(\eps)\OPT$. The disjointness of the $\bfe$ and $\bfd_k$ as well as the net size bounds carry over directly. Finally, the bounds on the coordinates of $\bfd_k$ follow from
        \begin{align*}
            H(\abs{\bfd_k(i)}) &\leq \abs*{\bfd_k(i)}^p \tag{$p\in[1,2]$} \\
            &\leq O(1)(\abs{\bfy(i)}^p + \abs{\bfv(i)}^p) \\
            &\leq O(1)\bracks*{\frac{\bfw_i^p(\bfA)}{d}(1+\eps^2)^{pk}\norm*{\bfy}_p^p + \kappa\frac{\overline{\bfs_i}^H(\bfA)\cdot(1+\eps^2)^{p(k+2)}}{\eps^4\cdot d}\OPT^2} \tag{$i\in B_{k,\bfy}$} \\
            &\leq O(1)\bracks*{\kappa\frac{\bfw_i^p(\bfA)}{d}(1+\eps^2)^{pk}\norm*{\bfy}_H^2 + \kappa\frac{\overline{\bfs_i}^H(\bfA)\cdot(1+\eps^2)^{p(k+2)}}{\eps^4\cdot d}\OPT^2} \\
            &= O(\kappa)\frac{\overline{\bfs_i}^H(\bfA)\cdot(1+\eps^2)^{pk}}{\eps^4\cdot d}\OPT^2 \\
        \end{align*}
        for $i\in B_{k,\bfy}$, and similarly for other cases as well as for $\bfe$.

        This completes the proof of Claim \ref{clm:huber-compact-rounding}.
    \end{proof}

    We return to proving Lemma \ref{lem:huber-additive2}. Recall that we reduced our task to proving the approximation guarantee Equation \eqref{eq:huber-additive2-guarantee} for all vectors $\bfr'$ belonging to an $O(\eps^2\rho)$-cover over the set $\mathcal B_\rho^H - \bar\bfz$. We will do so using the cover given by Claim \ref{clm:huber-compact-rounding}, with $\eps$ set to $\eps^2$. Furthermore, we set
    \[
        \overline{\bfs_i}^H(\bfA) \coloneqq \tilde\bfs_i^H(\bfA) + \sum_{p\in\mathcal I} \tilde\bfw_i^p(\bfA),
    \]
    i.e., the sum of all the approximate $\ell_p$ Lewis weights for $p\in \mathcal I$ as well as approximate Huber sensitivities $\tilde\bfs_i^H(\bfA)$. This indeed satisfies the hypothesis \eqref{eq:huber-lp-sensitivity-bound} of Claim \ref{clm:huber-compact-rounding}. 
    
    Then, performing a Bernstein bound gives the active version of Lemma \ref{lem:huber-bernstein}. 

    \begin{claim}\label{clm:huber-bernstein-active}
        Let $m = d\poly((\log n),\eps^{-1},\log(1/\delta))$ and $\kappa\geq 1$. Let $\bfw\geq\mathbf{1}_n$ be a set of weights chosen randomly so that
        \[
            \bfw_i \coloneqq \begin{cases}
                1/\bfp_i & \text{w.p. $\bfp_i$} \\
                0 & \text{otherwise}
            \end{cases}
        \]
        where
        \[
            \bfp_i \geq \min\braces*{1, m\cdot \kappa\bracks*{\frac1n + \frac{\overline{\bfs_i}^H(\bfA)}{d}}}
        \]
        Let
        \[
            S_\kappa \coloneqq \braces*{\bfy\in\mathcal V : \frac{\min_{p\in\mathcal I}\norm*{\bfy}_p^p}{\norm*{\bfy}_H^2}\leq \kappa}
        \]
        Then with probability at least $1 - \delta$, 
        \[
            \norm*{\bfy}_{H,\bfw} = (1\pm\eps)\norm*{\bfy}_H
        \]
        for all $\bfy\in \mathcal N\cap S_\kappa$, where $\mathcal N$ is an $\eps^2\rho$-net over $\mathcal B_\rho^H-\bfv$ given by Claim \ref{clm:huber-compact-rounding}, by setting $\eps$ in the lemma to $\eps^2$.
    \end{claim}
    \begin{proof}
        The proof follows that of Lemma \ref{lem:huber-bernstein} almost exactly, with minimal changes. The only necessary change is that the coordinate upper bounds of Claim \ref{clm:huber-compact-rounding} are now proportional to $\overline{\bfs_i}^H(\bfA)$ rather than $\bfw_i^p(\bfA)$. However, this is not a problem, since we are sampling with these probabilities, and thus does not change the proof. 
    \end{proof}
    
    Finally, be applying Corollary \ref{cor:generalized-huber-inequality} with $\gamma = 1$, we have the approximation guarantee of Claim \ref{clm:huber-bernstein-active} with $\kappa = n^{3-2\sqrt 2}$. 
    
    This completes the proof of Lemma \ref{lem:huber-additive2}.
\end{proof}

With the unweighted algorithm in hand, we can then obtain a weighted algorithm, and use it to obtain our recursive algorithm.

\begin{algorithm}
	\caption{Weighted Huber sampling}
	\textbf{input:} Matrix $\bfA \in \R^{n \times d}$ and weights $\bfw$. \\
	\textbf{output:} Weights $\bfw'$.
	\begin{algorithmic}[1] % The number tells where the line numbering should start
        \For{$j\in[O(\log(1+\norm*{\bfw}_\infty)/\eps)]$}
        \State $T_j\gets\{i\in[n] : (1+\eps)^{j-1} \leq \bfw_i < (1+\eps)^j\}$
        \State Run Algorithm \ref{alg:unweighted-huber-active} on $\bfA\mid_{T_j}$ to obtain weights $\bfw^{(j)}$
        \State Set $\bfw'_i = (1+\eps)^j\bfw^{(j)}_i$ for $i\in T_j$
        \EndFor
        \State \Return $\bfw'$
	\end{algorithmic}\label{alg:weighted-huber-active}
\end{algorithm}

\begin{algorithm}
	\caption{Recursive Huber sampling}
	\textbf{input:} Matrix $\bfA \in \R^{n \times d}$, weights $\bfw$ (defaulted to $\mathbf{1}_n$). \\
	\textbf{output:} Weights $\bfw''$.
	\begin{algorithmic}[1] % The number tells where the line numbering should start
        \If{$\nnz(\bfw) \leq O(d^{(1+\sqrt2)/2}\poly((\log n)/\eps))$}
            \State \Return $\bfw$
        \EndIf
        \State Obtain weights $\bfw'$ by running Algorithm \ref{alg:weighted-huber-active} on $\bfA$ with weights $\bfw$
        \State Obtain weights $\bfw''$ by recursively running Algorithm \ref{alg:huber-recursive-active} on $\bfA$ with weights $\bfw'$
        \State \Return $\bfw''$
	\end{algorithmic}\label{alg:huber-recursive-active}
\end{algorithm}


\begin{lemma}\label{lem:huber-additive2-weighted}
    Consider the setting of Lemma \ref{lem:huber-clip}. Suppose that $\bfw$ is obtained by performing one step of Algorithm \ref{alg:weighted-huber-active}. Then with probability at least $1-\delta$, for all $\bfx\in\mathbb R^{d}$ with $\norm*{\bfA\bfx}_{H} = O(\OPT)$,
    \begin{equation}
        \abs*{\norm*{\bfA\bfx-\bar\bfz}_{H,\bfw}^2 - \norm*{\bfA\bfx-\bar\bfz}_{H,\bfw'}^2} = O(\eps)\cdot\OPT^2.
    \end{equation}
    Furthermore, we have that
    \begin{itemize}
        \item $\norm*{\bfw'}_\infty \leq n\norm*{\bfw}_\infty$
        \item $\nnz(\bfw') \leq \log(\norm*{\bfw}_\infty)\nnz(\bfw)^{3-2\sqrt 2}\cdot\poly(\log n,\eps^{-1},\delta^{-1})$
    \end{itemize}
\end{lemma}
\begin{proof}
    This follows the same reasoning as the proof of Lemma \ref{lem:huber-one-recursive-step}, by applying the guarantees of Lemma \ref{lem:huber-additive2} to $(1+\eps)$-approximate level sets of weights.
\end{proof}

\begin{lemma}
    Let $\bfw\geq\mathbf{1}_n$ be a set of weights. Suppose that $\bfw'$ is obtained from running Algorithm \ref{alg:weighted-huber-active}. Let $\bar\bfx$ be an approximate minimizer such that
    \[
        \norm*{\bfA\bar\bfx-\bfz}_{H,\bfw'}^2 \leq (1+\eps)\min_{\bfx}\norm*{\bfA\bfx-\bfz}_{H,\bfw'}^2.
    \]
    Then, with probability at least $1-\delta$,
    \[
        \norm*{\bfA\bar\bfx - \bfz}_{H,\bfw}^2 \leq (1+ O(\eps/\delta))\min_\bfx\norm*{\bfA\bfx-\bfz}_{H,\bfw}^2
    \]
\end{lemma}
\begin{proof}
    Let $\bfA\bfx$ have $\norm*{\bfA\bfx}_{H,\bfw} = O(\OPT)$. By Lemma \ref{lem:huber-additive2-weighted},
    \[
        \norm*{(\bfA\bfx-\bfz)\mid_{\overline{\mathcal B}}}_{H,\bfw'}^2 = \norm*{(\bfA\bfx-\bfz)\mid_{\overline{\mathcal B}}}_{H,\bfw}^2 \pm O(\eps)\OPT^2.
    \]
    Furthermore, by Lemma \ref{lem:huber-clip},
    \[
        \norm*{(\bfA\bfx-\bfz)\mid_{\mathcal B}}_{H,\bfw}^2 = (1\pm\eps)\norm*{\bfz\mid_{\mathcal B}}_{H,\bfw}^2
    \]
    and similarly,
    \[
        \norm*{(\bfA\bfx-\bfz)\mid_{\mathcal B}}_{H,\bfw'}^2 = (1\pm\eps)\norm*{\bfz\mid_{\mathcal B}}_{H,\bfw'}^2
    \]
    By Markov's inequality, $\norm*{\bfz\mid_{\mathcal B}}_{H,\bfw'}^2 = O(\delta^{-1}\norm*{\bfz\mid_{\mathcal B}}_{H,\bfw}^2)$ with probability at least $1-\delta$. Then under this event,
    \begin{align*}
        \norm*{\bfA\bfx-\bfz}_{H,\bfw}^2 &= \norm*{\bfA\bfx-\bfz}_{H,\bfw'}^2 - \norm*{\bfz\mid_{\mathcal B}}_{H,\bfw'} + \norm*{\bfz\mid_{\mathcal B}}_{H,\bfw}^2 \pm O(\eps)(\OPT^2 + \norm*{\bfz\mid_{\mathcal B}}_{H,\bfw}^2 + \norm*{\bfz\mid_{\mathcal B}}_{H,\bfw'}^2) \\
        &= \norm*{\bfA\bfx-\bfz}_{H,\bfw'}^2 - \norm*{\bfz\mid_{\mathcal B}}_{H,\bfw'} + \norm*{\bfz\mid_{\mathcal B}}_{H,\bfw}^2 \pm O(\eps/\delta)(\OPT^2 + \norm*{\bfz\mid_{\mathcal B}}_{H,\bfw}^2) \\
        &= \norm*{\bfA\bfx-\bfz}_{H,\bfw'}^2 - \norm*{\bfz\mid_{\mathcal B}}_{H,\bfw'} + \norm*{\bfz\mid_{\mathcal B}}_{H,\bfw}^2 \pm O(\eps/\delta)\OPT^2.
    \end{align*}
    This gives the desired conclusion.
\end{proof}

Finally, we are ready to give the proof of the recursive algorithm. 


\begin{proof}[\textbf{Proof of Theorem \ref{thm:active-huber}}]
    Note that in Lemma \ref{lem:huber-additive2-weighted}, the number of samples is
    \[
        \log(\norm*{\bfw}_\infty)\nnz(\bfw)^{3-2\sqrt 2}d\poly(\log n,\eps^{-1},\log(1/\delta))
    \]
    at each recursive call. Furthermore, as long as we make at most $O(\log n)$ recursive calls, the weights have magnitude at most $\norm*{\bfw}_\infty \leq n^{O(\log n)}$ at all times. Thus, at each recursive call starting from $m$ rows, we reduce to
    \[
        m^{3-2\sqrt 2}d\poly(\log n,\eps^{-1},\log(1/\delta)).
    \]
    Now let $m_i$ be the number of nonzero rows after $i$ recursive calls, let $a_i = \log m_i$, and let $b = \log(d\poly(\log n,\eps^{-1},\log(1/\delta)))$. Then, the $a_i$ satisfy a recurrence
    \[
        a_{i+1} = (3-2\sqrt 2)a_i + b
    \]
    for $i \leq O(\log n)$. The closed form solution for this recurrence in Lemma \ref{lem:affine-recurrence} gives
    \begin{align*}
        a_i &= \frac{1}{1-(3-2\sqrt 2)} \parens*{b - \lambda^{i}\parens*{b - (1-\lambda) a_0}} \\
        &= \frac{1+\sqrt 2}{2} \parens*{b - \lambda^{i}\parens*{b - (1-\lambda) a_0}} \\
    \end{align*}
    Then, as discussed in the proof of Theorem \ref{thm:huber-subspace-embedding}, after at most $O(\log\log n)$ iterations, the number of rows is at most
    \[
        m_i = \exp(a_i) = O(\exp(b)^{(1+\sqrt2)/2}) = d^{(1+\sqrt 2)/2}\poly(\log n,\eps^{-1}).
    \]
\end{proof}
